From Flow to Fuse: A Cognitive Perspective

The concept of flow is used extensively in HCI, video games, and many other fields, but its prevalent definition is conceptually vague and alternative interpretations have contributed to ambiguity in the literature. To address this, we use cognitive science theory to expose inconsistencies in flow's prevalent definition, and introduce fuse, a concept related to flow but consistent with cognitive science, and defined as the "fusion of activity-related sensory stimuli and awareness". Based on this definition, we develop a preliminary model that hypothesizes fuse's underlying cognitive processes. To illustrate the model's practical value, we derive a set of design heuristics that we exemplify in the context of video games. Together, the fuse definition, model and design heuristics form our theoretical framework, and are a product of rethinking flow from a cognitive perspective with the purpose of improving conceptual clarity and theoretical robustness in the literature.

==> tables/table-example1.tex <==
\begin{table}%[htbp]
  \centering
  \caption{Results on the summative scales, in \textit{M} (\textit{SD}), across all three GeoExplorer versions.} 
    \begin{tabular}{lcccccccccccccccccc}
    \toprule
 & \textbf{Basic} & \textbf{Plus} & \textbf{Advanced} \\
\textbf{Scale} & \textit{n} = 29 & \textit{n} = 70 & \textit{n} = 207 \\
  \midrule
    CPT Learning & 3.98 (0.53) & 4.09 (0.56) & 3.96 (0.75) \\
    Integration & 3.74 (0.46) & 4.33 (0.65) & 3.94 (0.92) \\
    Geotechnical Learning & 3.75 (0.53) & 3.97 (0.62) & 3.73 (0.80) \\
    Career & 3.07 (0.93) & 3.15 (1.02) & 3.30 (0.99) \\
    Learning & 3.82 (0.49) & 3.97 (0.57) & 3.84 (0.70) \\
    \bottomrule
    \end{tabular}
  \label{tab:general}
\end{table}

\begin{table}%[htbp]
  \centering
  \caption{Routine Correlations} 
    \begin{tabular}{lcccccccccccccccccc}
    \toprule
 & \textbf{Practice} & \textbf{Sleep} & \textbf{Exercise} & \textbf{MHC-SF} & \textbf{PSS} & \textbf{Health} & \textbf{Days Training} \\
 \midrule
\textbf{Practice} & 1\\
 \textbf{Sleep} & -.1 & 1\\
 \textbf{Exercise} & -.05 & -.08 & 1\\
 \textbf{MHC-SF} & .19 & .01 & -.05 & 1\\
 \textbf{PSS} & -.08 & .08 & -.01 & -.63*** & 1\\
 \textbf{Health} & -.01 & .07 & .01 & .27 & -.24 & 1\\
 \textbf{Days Training} & .55*** & -.06 & -.13 & .27 & -.07 & .22 & 1\\

    \bottomrule
    \end{tabular}
  \label{tab:Routine}
\end{table} 



==> tables/table-example2.tex <==
\begin{table*}%[htbp]
  \centering
  \caption{Overview of the GeoExplorer-Advanced results (\textit{n} = 207) on all individual survey items, in \textit{Mdn} (\textit{IQR}).} 
  \begin{threeparttable}
  \setlength\tabcolsep{4pt} 
    %\small
    \begin{tabular}{clcccccc}
    \toprule
   &   & \multicolumn{2}{c}{\textbf{Gender}\tnote{a}} & \multicolumn{4}{c}{\textbf{Race/Ethnicity}\tnote{b}}\\
   &   & \multicolumn{2}{c}{(\textit{n} = 191)} & \multicolumn{4}{c}{(\textit{n} = 180)}  \\
   \cmidrule(r){3-4}\cmidrule(r){5-8}
    \textbf{Item } & \textbf{Description} & F & M  & A  & L  & W & O \\
  \midrule
     \multicolumn{2}{l}{\textit{CPT Learning} ($\alpha$ = .92)}\\% & 4.01 (0.78) & 3.96 (0.71)  & 4.06 (0.64) & 4.06 (0.85) & 3.93 (0.72) & 3.76 (0.96)\\
    1 & Learn about the operation of CPT equipment.  & 4 (4 - 5)  & 4 (4 - 4)    & 4 (4 - 4.75)  & 4 (4 - 5)     & 4 (4 - 4)  & 4 (3 - 4)\\
    
    2 & Visualize subsurface stratigraphy. & 4 (4 - 4.5)  & 4 (4 - 4)     & 4 (4 - 4)  & 4 (4 - 5)    & 4 (4 - 4)    & 4 (3 - 4)     \\
 
    3 & Simulate field conditions & 4 (4 - 4.5)  & 4 (4 - 4)     & 4 (4 - 4)  & 4 (4 - 5)     & 4 (4 - 4)  & 4 (3 - 4.5)     \\

    4 & \multicolumn{1}{p{25em}}{Conduct a geotechnical site investigation using\newline{} CPT equipment.} & 4 (4 - 4.5)  & 4 (4 - 4)    & 4 (4 - 4.75)    & 4 (4 - 5)    & 4 (4 - 4)    & 4 (3 - 4.5)\\[0.35cm]

    \multicolumn{2}{l}{\textit{Integration} ($\alpha$ = .94)} \\%& 4.04 (0.85) & 3.92 (0.94) & 3.92 (0.94) & 4.14 (0.80) & 4.11 (0.72) & 3.28 (1.28)\\
    5 & \multicolumn{1}{p{25em}}{The class lectures prepared me for conducting the\newline{}CPT in the mock internship.%\newline{}(i.e., using the appropriate methods and tools to collect data about soils). 
    } & 4 (4 - 5)  & 4 (4 - 5)     & 4 (3 - 5)  & 4 (4 - 5)     & 4 (4 - 5)  & 4 (2.5 - 4)\\

    6 & \multicolumn{1}{p{25em}}{The class lectures prepared me for analyzing\newline{} the results from the CPT.} & 4 (4 - 5)  & 4 (4 - 5)     & 4 (3.25 - 5)  & 4 (4 - 5)     & 4 (4 - 4.5)  & 3 (2.5 - 4) \\
    
    7 & \multicolumn{1}{p{25em}}{The CPT Environment was a good way to put what\newline{} I learned in class into practice.} & 4 (4 - 5)  & 4 (4 - 4.5)     & 4 (3 - 5)  & 4 (4 - 5)     & 4 (4 - 5)  & 4 (3 - 4) \\[0.35cm]
    
    \multicolumn{2}{l}{\textit{Geotechnical Learning} ($\alpha$ = .90)}\\%  & 3.71 (0.84) & 3.80 (0.72) & 3.98 (0.70) & 3.76 (0.86) & 3.69 (0.74) & 3.61 (0.90) \\
    8 & Helped me understand geotechnical engineering better. & 4 (3 - 4)  & 4 (4 - 4)     & 4 (4 - 4)  & 4 (3 - 4)     & 4 (4 - 4)  & 4 (3 - 4)   \\

    9 & Made me want to learn more about geotechnical engineering. & 4 (3 - 4)  & 4 (3 - 4)     & 4 (3 - 4)  & 4 (3 - 4)    & 4 (3 - 4)      & 3 (3 - 4)     \\

    10 & Helped show me why geotechnical engineering is important. & 4 (3 - 4)  & 4 (3 - 4)     & 4 (3 - 5)  & 4 (4 - 4)     & 4 (3 - 4)  & 3.5 (3 - 4)      \\

    11 & \multicolumn{1}{p{25em}}{Was an effective way to learn about site investigation methods \newline{}that are relevant to geotechnical engineering.} & 4 (3.5 - 4.5)  & 4 (4 - 4)     & 4 (4 - 4)  & 4 (3 - 4)     & 4 (4 - 4)  & 4 (3 - 4)     \\[0.35cm]
 
    \multicolumn{2}{l}{\textit{Career} ($\alpha$ = .94)} \\% & 3.28 (1.16) & 3.34 (0.89) & 3.18 (1.08) & 3.47 (0.88) & 3.28 (1.03) & 3.30 (0.90)\\
    12 & Take more classes that focus on geotechnical engineering. & 4 (3 - 4)  & 4 (3 - 4)     & 3 (2 - 4)  & 4 (3 - 4)    & 3.5 (3 - 4)    & 4 (3 - 4)\\
    
    13 & Pursue a concentration in geotechnical engineering. & 3 (2.5 - 4)  & 3 (3 - 4)     & 3 (2 - 4)  & 3 (3 - 4)    & 3 (3 - 4)    & 3 (3 - 4)     \\

    14 & Pursue a graduate degree in geotechnical engineering. & 3 (2 - 4)  & 3 (3 - 4)    & 3 (2 - 4)    & 3 (3 - 4)    & 3 (2 - 4)    & 3 (3 - 4)     \\

    15 & Seek employment with a geotechnical engineering firm. & 3 (3 - 4)  & 3 (3 - 4)     & 3 (2 - 4)  & 4 (3 - 4)    & 3 (3 - 4)    & 3 (3 - 4)     \\%[0.5cm]
     %\multicolumn{2}{l}{\textit{Learning}\tnote{c} ($\alpha$ = .88)}  & 3.85 (0.73) & 3.86 (0.66) & 4.01 (0.64) & 3.90 (0.81) & 3.79 (0.61)  & 3.69 (0.92)\\
    \bottomrule
    \end{tabular}
    \smallskip
    \scriptsize
    \begin{tablenotes}
        \scriptsize 
        \item \textit{Gender}: F = Female; M = Male. \textit{Race/Ethnicity}: A = Asian; L = Latino/Latina or Hispanic; W = Caucasian or White; O = other race/ethnicity.
        %\item[c] Learning is a scale that combines the items of the CPT Learning and Geotechnical Engineering Learning scales minus Items 1 and 8. 
    \end{tablenotes}
  \end{threeparttable}
    \label{tab:individual}
\end{table*}
